A Practical Distributed Universal Construction with Unknown Participants

Modern distributed systems employ atomic read-modify-write primitives to coordinate concurrent operations. Such primitives are typically built on top of a central server, or rely on an agreement protocol. Both approaches provide a universal construction, that is, a general mechanism to construct atomic and responsive objects. These two techniques are however known to be inherently costly. As a consequence, they may result in bottlenecks in applications using them for coordination. In this paper, we investigate another direction to implement a universal construction. Our idea is to delegate the implementation of the universal construction to the clients, and solely implement a distributed shared atomic memory at the servers side. The construction we propose is obstruction-free. It can be implemented in a purely asynchronous manner, and it does not assume the knowledge of the participants. It is built on top of grafarius and racing objects, two novel shared abstractions that we introduce in detail. To assess the benefits of our approach, we present a prototype implementation on top of the Cassandra data store, and compare it empirically to the Zookeeper coordination service.

==> Makefile <==
FILE=paper
FINAL=sutra-submission-

MAKEFLAGS=	--no-print-directory

# GNUPlot source files
GPSOURCE= 

# EPS files included
EPSSOURCE= 

# BIB files included
BIBS=

# .tex file includes or inputs
TEXIN= \
	paper.tex

# other file dependencies
DEPS= Makefile \
	macros.sty

# Output assumed to depend on $FILE, $TEXIN, $GPSOURCE, $EPSSOURCE, $BIBS and $DEPS


GRAPHICSSOURCE= ${GPSOURCE} ${EPSSOURCE} 

EPSGRAPHICS= $(GPSOURCE:.gp=.eps) ${EPSSOURCE}

PDFGRAPHICS=$(EPSGRAPHICS:.eps=.pdf)

GNUPLOT= gnuplot 

default: pdf

${FINAL}.pdf ${FINAL}.ps.gz final: ${FILE}.dvi
	${MAKE} bib
	pdflatex --interaction nonstopmode ${FILE}
	pdflatex --interaction nonstopmode ${FILE}


tags etags: TAGS

TAGS: ${FILE}.tex ${TEXIN} ${DEPS}
	etags ${FILE}.tex ${TEXIN} ${DEPS}

graphics: epsgraphics pdfgraphics

epsgraphics: ${EPSGRAPHICS}

pdfgraphics: ${PDFGRAPHICS}

dvi: $(FILE).dvi 

# $(FILE).dvi ${FILE}.aux: ${FILE}.tex ${DEPS} ${EPSGRAPHICS}
# 	rm -f ${FILE}.ps ${FILE}.ps.gz ${FILE}.pdf
# 	latex $(FILE)
# 	latex $(FILE)

pdf: $(FILE).pdf 
	${MAKE} bib
	pdflatex --interaction nonstopmode ${FILE}
	pdflatex --interaction nonstopmode ${FILE}

$(FILE).pdf: ${FILE}.tex ${TEXIN} ${DEPS} ${PDFGRAPHICS}
	pdflatex --interaction nonstopmode $(FILE)

force: default bib
	rm -f ${FILE}.dvi ${FILE}.pdf; ${MAKE} default

${FILE}.bbl: ${FILE}.aux ${BIBS} 
		BIBINPUTS=tmp/:$$BIBINPUTS bibtex $(FILE)
		sed -e 's/%//g' < $(FILE).bbl > $(FILE).bbl~
		mv $(FILE).bbl~ $(FILE).bbl

clean::
	rm -rf tmp/

bib: $(FILE).bbl 

figs:
	gnuplot results/cas/different/different.plot 
	gnuplot results/cas/same/same.plot
	gnuplot results/lock/same.plot

clean::
		/bin/rm -f f *~ *.bak *.aux *.log *.toc *.lof *.dvi *.bbl *.blg *.out *.pdf

spotless:	clean
		/bin/rm -f *.dvi *.ps *.ps.gz *.pdf

ps: $(FILE).ps

# pdflatex: $(FILE).pdf

# $(FILE).pdf $(FILE).aux: ${FILE}.tex ${PDFGRAPHICS}
# 	pdflatex ${FILE}.tex

gz ps.gz: $(FILE).ps.gz

print lpr: $(FILE).ps
	lpr $(FILE).ps || gsprint $(FILE).ps

gv: $(FILE).ps
	gv -nopixmap $(FILE).ps

$(FILE).dvi: $(FILE).tex $(FIGS)

%.prn: %.ppt
	@echo 'You must manually create $@ from Powerpoint $^!' 2>&1; exit 1
clean::
	rm -f *.prn

%.eps: %.obj
	tgif -print -eps $^
%.eps: %.gp
	$(GNUPLOT) $^
# %.eps: %.gp dat/%.dat
#	$(GNUPLOT) $^
%.eps: %.fig
	fig2dev -L eps $^ >$@
%.eps: %.prn
	ps2epsi $^ $@
clean::
	rm -f ${EPSGRAPHICS}

%.eps: %.dia
	dia -e $@ $^
# %.eps: %.ps
#	ps2epsi $^ $@
%.eps: %.epsraw
	ps2epsi $^ $@
clean::
	rm -f *.eps

%.dvi: %.tex
	latex $^

# According to ACM instructions, '-P cmz' embeds Type 1 fonts, which
# enables later PDF generation to be of higher quality 
%.ps: %.dvi
	dvips -C a4 -P cmz $^ -o
	rm -f $@.gz
%.ps.gz: %.ps
	gzip --best $^

%.pdf: %.tex
	${MAKE} bib
	pdflatex --interaction nonstopmode ${FILE}
	pdflatex --interaction nonstopmode ${FILE}

clean::
	rm -f ${PDFGRAPHICS}

# subalgorithms
sub1.prn sub2.prn sub3.prn sub4.prn sub5.prn: subalgorithms.ppt
	@echo 'You must manually create $@ from Powerpoint $^!' 2>&1; exit 1
pdffigs.tgz: ${PDFGRAPHICS}
	tar czf pdffigs.tgz ${PDFGRAPHICS}
epsfigs.tgz: ${EPSGRAPHICS}
	tar czf epsfigs.tgz ${EPSGRAPHICS}

tgz: ${FINAL}.pdf
	dir=`basename $$PWD`; \
	tar czvf $(FILE).tgz -C .. \
	$(patsubst %,$$dir/%,\
	    ${FILE}.tex \
	    ${TEXIN} \
	    ${DEPS} \
	    ${EPSSOURCE} \
	    ${GPSOURCE} \
	    ${patsubst %,dat/%,${GPSOURCE:.gp=.dat}}\
	    ${BIBS} \
	    ${FINAL}.pdf \
	)

update:
	svn update

commit:
	svn commit -m ''


==> results/lock/different.tex <==
% GNUPLOT: LaTeX picture
\setlength{\unitlength}{0.240900pt}
\ifx\plotpoint\undefined\newsavebox{\plotpoint}\fi
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\begin{picture}(750,540)(0,0)
\sbox{\plotpoint}{\rule[-0.200pt]{0.400pt}{0.400pt}}%
\put(171.0,104.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,104){\makebox(0,0)[r]{ 200}}
\put(669.0,104.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,160.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,160){\makebox(0,0)[r]{ 250}}
\put(669.0,160.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,217.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,217){\makebox(0,0)[r]{ 300}}
\put(669.0,217.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,273.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,273){\makebox(0,0)[r]{ 350}}
\put(669.0,273.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,330.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,330){\makebox(0,0)[r]{ 400}}
\put(669.0,330.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,386.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,386){\makebox(0,0)[r]{ 450}}
\put(669.0,386.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,443.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,443){\makebox(0,0)[r]{ 500}}
\put(669.0,443.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(171.0,499.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(151,499){\makebox(0,0)[r]{ 550}}
\put(669.0,499.0){\rule[-0.200pt]{4.818pt}{0.400pt}}
\put(275,104){\usebox{\plotpoint}}
\put(275,84){\makebox(0,0)[l]{Zk}}
\put(378,104){\usebox{\plotpoint}}
\put(378,84){\makebox(0,0)[l]{3}}
\put(482,104){\usebox{\plotpoint}}
\put(482,84){\makebox(0,0)[l]{6}}
\put(585,104){\usebox{\plotpoint}}
\put(585,84){\makebox(0,0)[l]{12}}
\put(171.0,104.0){\rule[-0.200pt]{0.400pt}{95.155pt}}
\put(171.0,104.0){\rule[-0.200pt]{124.786pt}{0.400pt}}
\put(689.0,104.0){\rule[-0.200pt]{0.400pt}{95.155pt}}
\put(171.0,499.0){\rule[-0.200pt]{124.786pt}{0.400pt}}
\put(30,301){\makebox(0,0){\rotatebox{90}{\footnotesize Throughput (ops/s)}}}
\put(430,29){\makebox(0,0){\#Servers}}
\put(259.0,104.0){\rule[-0.200pt]{0.400pt}{85.519pt}}
\put(259.0,459.0){\rule[-0.200pt]{15.899pt}{0.400pt}}
\put(325.0,104.0){\rule[-0.200pt]{0.400pt}{85.519pt}}
\put(259.0,104.0){\rule[-0.200pt]{15.899pt}{0.400pt}}
\put(363.0,104.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(363.0,124.0){\rule[-0.200pt]{15.658pt}{0.400pt}}
\put(428.0,104.0){\rule[-0.200pt]{0.400pt}{4.818pt}}
\put(363.0,104.0){\rule[-0.200pt]{15.658pt}{0.400pt}}
\put(466.0,104.0){\rule[-0.200pt]{0.400pt}{14.213pt}}
\put(466.0,163.0){\rule[-0.200pt]{15.899pt}{0.400pt}}
\put(532.0,104.0){\rule[-0.200pt]{0.400pt}{14.213pt}}
\put(466.0,104.0){\rule[-0.200pt]{15.899pt}{0.400pt}}
\put(570.0,104.0){\rule[-0.200pt]{0.400pt}{41.676pt}}
\put(570.0,277.0){\rule[-0.200pt]{15.658pt}{0.400pt}}
\put(635.0,104.0){\rule[-0.200pt]{0.400pt}{41.676pt}}
\put(570.0,104.0){\rule[-0.200pt]{15.658pt}{0.400pt}}
\put(171.0,104.0){\rule[-0.200pt]{0.400pt}{95.155pt}}
\put(171.0,104.0){\rule[-0.200pt]{124.786pt}{0.400pt}}
\put(689.0,104.0){\rule[-0.200pt]{0.400pt}{95.155pt}}
\put(171.0,499.0){\rule[-0.200pt]{124.786pt}{0.400pt}}
\end{picture}


==> same.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(3960.00,3528.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(814,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(814,874){\makebox(0,0)[r]{\strut{} 10}}%
      \put(814,1044){\makebox(0,0)[r]{\strut{} 20}}%
      \put(814,1214){\makebox(0,0)[r]{\strut{} 30}}%
      \put(814,1383){\makebox(0,0)[r]{\strut{} 40}}%
      \put(814,1553){\makebox(0,0)[r]{\strut{} 50}}%
      \put(814,1723){\makebox(0,0)[r]{\strut{} 60}}%
      \put(946,484){\makebox(0,0){\strut{} 0}}%
      \put(1600,484){\makebox(0,0){\strut{} 5}}%
      \put(2254,484){\makebox(0,0){\strut{} 10}}%
      \put(2909,484){\makebox(0,0){\strut{} 15}}%
      \put(3563,484){\makebox(0,0){\strut{} 20}}%
      \put(176,1213){\rotatebox{-270}{\makebox(0,0){\strut{}\rotatebox{90}{\scriptsize Latency (ms)}}}}%
      \put(2254,154){\makebox(0,0){\strut{} {\scriptsize \# Clients}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(2487,3354){\makebox(0,0)[r]{\strut{}$M_{approx}=10$}}%
      \csname LTb\endcsname%
      \put(2487,3134){\makebox(0,0)[r]{\strut{}$M_{approx}=20$}}%
      \csname LTb\endcsname%
      \put(2487,2914){\makebox(0,0)[r]{\strut{}$M_{approx}=40$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{same}}%
    \gplfronttext
  \end{picture}%
\endgroup

